Improving End-to-End Text Image Translation From the Auxiliary Text Translation Task

End-to-end text image translation (TIT), which aims at translating the source language embedded in images to the target language, has attracted intensive attention in recent research. However, data sparsity limits the performance of end-to-end text image translation. Multi-task learning is a non-trivial way to alleviate this problem via exploring knowledge from complementary related tasks. In this paper, we propose a novel text translation enhanced text image translation, which trains the end-to-end model with text translation as an auxiliary task. By sharing model parameters and multi-task training, our model is able to take full advantage of easily-available large-scale text parallel corpus. Extensive experimental results show our proposed method outperforms existing end-to-end methods, and the joint multi-task learning with both text translation and recognition tasks achieves better results, proving translation and recognition auxiliary tasks are complementary.

==> Fig_Tab/comparison_size_speed.tex <==
\begin{table}[t]
%\small
\centering
%\setlength{\belowcaptionskip}{-0.25cm}
%\setlength{\tabcolsep}{0.5mm}{
\caption{Comparison of cascaded and our end-to-end model on Zh$\Rightarrow$En translation direction.}
\begin{tabular}{c|c|c|c}
\toprule[0.4mm]
%\multirow{2}{*}{Architecture}		& \multicolumn{2}{c|}{En$\Rightarrow$Zh} & \multicolumn{2}{c|}{En$\Rightarrow$De} & \multicolumn{2}{c}{Zh$\Rightarrow$En}  \\
Architecture & BLEU ($\uparrow$) & Parameters ($\downarrow$) & Decoding Time ($\downarrow$) \\
%\cline{2-7}
\hline
%& Params. & Speed & Params. & Speed & Params. & Speed \\
%\hline
%\hline
{Cascaded} & 15.12 & 225 million & 0.21 seconds/sent \\
{Our Method} & 15.69 & 137 million & 0.11 seconds/sent \\
\bottomrule[0.4mm]
\end{tabular}
%}

\label{tab:comparison_size_speed}
\end{table}


%%% Previous

%\begin{table}[t]
%\small
%\centering
%\setlength{\tabcolsep}{0.35mm}{
%\begin{tabular}{c|cc|cc|cc}
%\toprule[0.4mm]
%\multirow{2}{*}{Architecture}		& \multicolumn{2}{c|}{En$\Rightarrow$Zh} & \multicolumn{2}{c|}{En$\Rightarrow$De} & \multicolumn{2}{c}{Zh$\Rightarrow$En}  \\
%\cline{2-7}
%& Params. & Speed & Params. & Speed & Params. & Speed \\
%%\hline
%\hline
%\textbf{Cascaded} & 195M & 0.33 & 179M & 0.38 & 225M & 0.21 \\
%\textbf{MATE-TIMT} & 122M & 0.19 & 114M & 0.23 & 137M & 0.11 \\
%\bottomrule[0.4mm]
%\end{tabular}
%}
%\caption{Comparison of modal size and decoding speed. Params. represents model parameters and unit for parameters is million ($\times 10^6$). Speed means the average time of decoding one sentence and the unit is second.}
%\label{tab:comparison_size_speed}
%\end{table}

==> Fig_Tab/fig_details_image_encoder.tex <==
\begin{figure}[t]
	\centering
%	\includegraphics[scale=0.36]{./overall_workflow-20210909-pipeline-e2e.pdf}
%	\includegraphics[scale=0.13]{./Figure_2.jpg}
%	\includegraphics[scale=0.65]{./details_of_MATE-TIMT-20210128.pdf}
	\includegraphics[scale=0.89]{./details_image_encoder-2021-01-17.pdf}
	\caption{Diagram of image encoder in our proposed end-to-end text image translation model.}
	\label{fig:details_image_encoder}       % Give a unique label
\end{figure}

==> Fig_Tab/fig_joint_multi_task.tex <==
\begin{figure}[t]
	\centering
%	\includegraphics[scale=0.36]{./overall_workflow-20210909-pipeline-e2e.pdf}
%	\includegraphics[scale=0.13]{./Figure_2.jpg}
%	\includegraphics[scale=0.65]{./details_of_MATE-TIMT-20210128.pdf}
	\includegraphics[scale=0.89]{./joint_multi_task-20211116.pdf}
	\caption{Illustration of joint multi-task architecture.}
	\label{fig:details_joint_multi_task}       % Give a unique label
\end{figure}

==> Fig_Tab/fig_multi_task_ocr_mt.tex <==
\begin{figure}[t]
	\centering
	
	\includegraphics[scale=0.48]{./multitask_ocr_mt-20211116.jpg}	
	\caption{Comparison of different multi-task settings. E2E denotes our proposed end-to-end backbone model, which consists of image encoder and transformer as shown in Figure (2).}
	\label{fig:multi_task_ocr_mt}       % Give a unique label
\end{figure}

==> Fig_Tab/fig_text_shapes.tex <==
\begin{figure*}[t]
	\centering
%	\includegraphics[scale=0.36]{./overall_workflow-20210909-pipeline-e2e.pdf}
%	\includegraphics[scale=0.13]{./Figure_2.jpg}
%	\includegraphics[scale=0.65]{./details_of_MATE-TIMT-20210128.pdf}
	\includegraphics[scale=0.23]{./fig_text_shapes-20211115.pdf}
	\caption{Examples of text image effects.}
	\label{fig_text_shape}       % Give a unique label
\end{figure*}

==> Fig_Tab/tab_cascaded_mt.tex <==
\begin{table}[h]
\small
\centering
\setlength{\tabcolsep}{3.5mm}{
\caption{BLEU score of MT models in OCR-MT cascaded models.}
\begin{tabular}{c|c|c|c}
\toprule[0.4mm]
%\multirow{2}{*}{Architecture}		& \multicolumn{2}{c|}{En$\Rightarrow$Zh} & \multicolumn{2}{c|}{En$\Rightarrow$De} & \multicolumn{2}{c}{Zh$\Rightarrow$En}  \\
Architecture & En$\Rightarrow$Zh & En$\Rightarrow$De & Zh$\Rightarrow$En  \\
%\cline{2-7}
\specialrule{0em}{0.50pt}{0.50pt}
\hline
\specialrule{0em}{0.50pt}{0.50pt}
%& Params. & Speed & Params. & Speed & Params. & Speed \\
%\hline
%\hline
%TPS+ResNet+BiLSTM+Attn. & 35.51\% & 29.54\% \\
Transformer & 25.38 & 20.97 & 17.56 \\
\bottomrule[0.4mm]
\end{tabular}
}

\label{tab:cascaded_mt}
\end{table}


%%% Previous

%\begin{table}[t]
%\small
%\centering
%\setlength{\tabcolsep}{0.35mm}{
%\begin{tabular}{c|cc|cc|cc}
%\toprule[0.4mm]
%\multirow{2}{*}{Architecture}		& \multicolumn{2}{c|}{En$\Rightarrow$Zh} & \multicolumn{2}{c|}{En$\Rightarrow$De} & \multicolumn{2}{c}{Zh$\Rightarrow$En}  \\
%\cline{2-7}
%& Params. & Speed & Params. & Speed & Params. & Speed \\
%%\hline
%\hline
%\textbf{Cascaded} & 195M & 0.33 & 179M & 0.38 & 225M & 0.21 \\
%\textbf{MATE-TIMT} & 122M & 0.19 & 114M & 0.23 & 137M & 0.11 \\
%\bottomrule[0.4mm]
%\end{tabular}
%}
%\caption{Comparison of modal size and decoding speed. Params. represents model parameters and unit for parameters is million ($\times 10^6$). Speed means the average time of decoding one sentence and the unit is second.}
%\label{tab:comparison_size_speed}
%\end{table}
